FPGA-Based Near-Memory Acceleration of Modern Data-Intensive Applications

Modern data-intensive applications demand high computation capabilities with strict power constraints. Unfortunately, such applications suffer from a significant waste of both execution cycles and energy in current computing systems due to the costly data movement between the computation units and the memory units. Genome analysis and weather prediction are two examples of such applications. Recent FPGAs couple a reconfigurable fabric with high-bandwidth memory (HBM) to enable more efficient data movement and improve overall performance and energy efficiency. This trend is an example of a paradigm shift to near-memory computing. We leverage such an FPGA with high-bandwidth memory (HBM) for improving the pre-alignment filtering step of genome analysis and representative kernels from a weather prediction model. Our evaluation demonstrates large speedups and energy savings over a high-end IBM POWER9 system and a conventional FPGA board with DDR4 memory. We conclude that FPGA-based near-memory computing has the potential to alleviate the data movement bottleneck for modern data-intensive applications.

==> Algorithms/cosmo.tex <==
\begin{algorithm}[h]
\scriptsize
\SetAlgoLined
\DontPrintSemicolon
\SetNoFillComment
\caption{Pseudo-code for vertical advection and horizontal diffusion kernels used by the COSMO~\cite{doms1999nonhydrostatic} weather prediction model.}
\label{algo:hdiffKernel}
% \caption{Pseudo-code for vertical advection
% used by the COSMO~\cite{doms1999nonhydrostatic} atmospheric model}
\label{algo:hdiffKernel}
\SetKwFunction{FMain}{verticalAdvection}
   \SetKwFunction{FTest}{forwardSweep}
    \SetKwFunction{FBack}{backwardSweep}
\SetKwProg{Fn}{Function}{}{end}
  
  \Fn{\FMain{float* ccol,
                float* dcol,
                float* wcon,
                float* ustage,
                float* upos,
                float* utens,
                float* utensstage
           }}{
       
             \For{$c\gets2$ \KwTo $column-2$}{
                    \For{$r\gets2$ \KwTo row-2}{
                    
               \Fn{\FTest{float* ccol,
                float* dcol,
                float* wcon,
                float* ustage,
                float* upos,
                float* utens,
                float* utensstage}} { 
                    \For{$d\gets1$ \KwTo $depth$}{
                       \tcc*[l]{forward sweep calculation}
                       }
                     }   
                       
                \Fn{\FBack{float* ccol,
                float* dcol,
                float* wcon,
                float* ustage,
                float* upos,
                float* utens,
                float* utensstage}} { 
                    \For{$d\gets depth-1$ \KwTo$ 1$}{
                       \tcc*[l]{backward sweep calculation}}}
                    }
                  }
            
               
   
         
}

% \end{algorithm}


% \vspace{-1cm}
% \begin{algorithm}
% \SetAlgoLined
% \DontPrintSemicolon
% \SetNoFillComment
\hline
% \caption{Pseudo-code for horizontal diffusion
% used by the COSMO~\cite{doms1999nonhydrostatic} atmospheric model}
% \label{algo:hdiffKernel}
\SetKwFunction{FMain}{horizontalDiffusion}
\SetKwProg{Fn}{Function}{}{end}
  
  \Fn{\FMain{float* src, float* dst}}{
       \For{$d\gets1$ \KwTo $depth$}{
             \For{$c\gets2$ \KwTo $column-2$}{
                    \For{$r\gets2$ \KwTo row-2}{
                        \tcc*[l]{\gagan{L}aplacian calculat\gagan{ion}}
                        $lap_{CR}=laplaceCalculate(c,r)$
                        \tcc{row-laplacian}
                        $lap_{CRm}=laplaceCalculate(c,r-1)$\;      
                        $lap_{CRp}=laplaceCalculate(c,r+1)$
                        \tcc{column-laplacian}
                        $lap_{CmR}=laplaceCalculate(c-1,r)$\;
                        $lap_{CpR}=laplaceCalculate(c+1,r)$
                        \tcc{column-flux calculat\gagan{ion}}\
                        $flux_{C} = lap_{CpR} - lap_{CR}$\;
                        $flux_{Cm} = lap_{CR} - lap_{CmR}$\;
                        \tcc{row-flux calculat\gagan{ion}}
                        $flux_{R} = lap_{CRp} - lap_{CR}$\;
                        $flux_{Rm} = lap_{CR} - lap_{CmR}$\;
                        \tcc{output calculat\gagan{ion}}
                        $dest[d][c][r] = src[d][c][r] -\\ 
                            c1 * (flux_{CR}- flux_{CmR}) + (flux_{CR}- flux_{CRm})$
                        }
            
                }
   
         }
}
\end{algorithm}



